Hierarchical approach to classify food scenes in egocentric photo-streams

Recent studies have shown that the environment where people eat can affect their nutritional behaviour. In this work, we provide automatic tools for a personalised analysis of a person's health habits by the examination of daily recorded egocentric photo-streams. Specifically, we propose a new automatic approach for the classification of food-related environments, that is able to classify up to 15 such scenes. In this way, people can monitor the context around their food intake in order to get an objective insight into their daily eating routine. We propose a model that classifies food-related scenes organized in a semantic hierarchy. Additionally, we present and make available a new egocentric dataset composed of more than 33000 images recorded by a wearable camera, over which our proposed model has been tested. Our approach obtains an accuracy and F-score of 56\% and 65\%, respectively, clearly outperforming the baseline methods.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> bayesian_example.tex <==
In order to understand the behaviour of the BSN model, we illustrate a simple example. Let us imagine that we have the semantic tree in Fig. \ref{fig:baynet}, and that we want to classify an egocentric image belonging to the class \textit{dining room}. In order to classify the given image, we compute the probability of the images belonging to the classes at the different levels of the semantic tree. First, we obtain the classification probabilities of the classes $P(eating)$, $P(shopping)$, and $P(preparing)$, corresponding to categories in Level 1 of the semantic tree (see Fig. \ref{fig:baynet}). In the second step, we obtain the classification probabilities with respect to the classes in Level 2. Finally, the probabilities of the classes included in  Level 3.  Our sample image describes the class \textit{dining room}. Thus, from the different levels classifications, we expect that the highest probabilities correspond to the category \textit{eating}, $P(indoor|eating)$ and $P(dining room|indoor)$, at Level 1, Level 2 and Level 3, respectively. 


Let us consider classes $C^i$ and $C^{i-1}$ so that subindex shows the level of the class in the hierarchy and $C^{i-1}$ is parent of $C^i$ in the higher level in the hierarchical organization of the tree.  

\begin{equation}
\resizebox{.3\textwidth}{!} 
{
$P(Q|C^{i-1}) = \frac{P(C^{i-1}|C^i)*P(C^i)}{P(C^{i-1})}$
}
\end{equation} or
\begin{equation}
\resizebox{.3\textwidth}{!} 
{
$P(C^i) = \frac{P(C^i|C^{i-1})*P(C^{i-1})}{P(C^{i-1}|C^i)}$
}
\end{equation}
Note that we can estimate $P(Q|C^{i-1})$ from the classifier of the network trained to classify the classes children of class $Q$, $P(C^{i-1}|C^i)$ is 1 since $C^i$ is a subclass of $C^{i-1}$  and $P(C^{i-1})$ is recursively estimated by applying the Bayes rule on $C^{i-1}$ and its class parent. 
\begin{equation}
\resizebox{.3\textwidth}{!} 
{
$P(C^i) = P(C^i|C^{i-1})*P(C^{i-1})$
}
\end{equation}
Applying recursively the Bayes rule, we obtain that 
\begin{equation}
\resizebox{.4\textwidth}{!} 
{
$P(C^i) = \Pi_{j=1}`^i P(C^j|C^{j-1})*P(C^{j-1})$
}
\end{equation}
Without loss of generality, we consider that the probability of the class in the root is 1 ($P(C^0)$). 

\textcolor{red}{De hecho esto es falso!!!! Para que sea aplicable, no necesitamos en la raiz un clasificador de food-related vs no food related?}

\textcolor{red}{Dejar numeros solo en las ecuaciones que se citan}

Let us illustrate this process on an example:
%\noindent At the same time, following the semantic tree, we know that:
\begin{equation}
\resizebox{.3\textwidth}{!} 
{
$P(indoor|eating) = \frac{P(eating|indoor)*P(indoor)}{P(eating)}$
}
\end{equation}
\begin{equation}
\resizebox{.3\textwidth}{!} 
{
$P(indoor) = \frac{P(eating)*P(indoor|eating)}{P(eating|indoor)}$
}
\end{equation}


Following the Bayes' theorem, we state that:
\begin{equation}
\resizebox{.4\textwidth}{!} 
{
$P(dining room|indoor) = \frac{P(indoor|dining room)*P(dining room)}{P(indoor)}$
}
\end{equation}
\begin{equation}
\resizebox{.3\textwidth}{!} 
{
$P(dining room) = \frac{P(indoor)*P(dining room|indoor)}{P(indoor|dining room)}$
}
\end{equation}
\noindent At the same time, following the semantic tree, we know that:
\begin{equation}
\resizebox{.3\textwidth}{!} 
{
$P(indoor|eating) = \frac{P(eating|indoor)*P(indoor)}{P(eating)}$
}
\end{equation}
\begin{equation}
\resizebox{.3\textwidth}{!} 
{
$P(indoor) = \frac{P(eating)*P(indoor|eating)}{P(eating|indoor)}$
}
\end{equation}

\noindent Thus, we can combine the probabilities and get the following equation that relates the probability of the events occurring,
\begin{equation}
\resizebox{.45\textwidth}{!} 
{
$P(dining room) =  \frac{P(dining room|indoor)*P(eating)*P(indoor|eating)}{P(eating|indoor)*P(indoor|dining room)}$
}
\end{equation}
 
%%%%
\noindent By having a look at the semantic tree defined, we know that \textit{indoor} relates to \textit{eating}, as \textit{dining room} relates to \textit{indoor eating}. Therefore, $P(eating|indoor)$ and $P(indoor|diningRoom)$ are equal to $1$. The probability of Dining Room occurring can be computed as:
\begin{equation}
\resizebox{.5\textwidth}{!} 
{
$P(dining room) =  P(dining room|indoor)*P(eating)*P(indoor|eating)$
}
\end{equation}

\begin{comment}
Furthermore, following this methodology we could assume and analyse several other aspects. For instance, we could go further and infer the probability of being at home eating as $P(home)$:
\begin{equation}
\resizebox{.3\textwidth}{!} 
{
$P(home|diningR) = \frac{P(diningR|home)*P(home)}{P(diningR)} = $
}
\end{equation}
\begin{equation}
\resizebox{.3\textwidth}{!} 
{
$\quad = P(home|diningR)*P(diningR|indoor)*P(indoor) $
}
\end{equation}
\end{comment}

To summarize, given an image our proposed BSN model computes the final classification by combining the obtained classification probabilities at the different levels of the defined semantic tree, following the Bayes’ theorem. 


==> bibliographies.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/foto_perfil_EstefaniaTalavera.png}}]{Estefania Talavera}
received her BSc degree in electronic engineering from Balearic Islands University in 2012 and her MSc degree in biomedical engineering from Polytechnic University of Catalonia in 2014. She is currently a PhD student at the University of Barcelona and University of Groningen. Her research interests are lifelogging and health applications.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/foto_maria.jpg}}]{María Leyva} received her BSc degree in Software Engineering from the University of Oviedo in 2011. She continued her studies with the MSc in Artificial Intelligence in the Polytechnic University of Catalonia, graduating in 2017. She is currently a PhD Student at the Johann Bernoulli Institute for Mathematics and Computer Science in the University of Groningen. \end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/Petia-foto.jpg}}]{Mostafa Kamal}
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/NicolaiPetkov.png}}]{Prof. Nicolai Petkov} received Dr.sc.techn. degree in Computer Engineering (Informationstechnik) from Dresden University of Technology, Dresden, Germany. Since 1991, he is professor of computer science and head of the Intelligent Systems group. His current research is in pattern recognition, machine learning, data analytics and brain-inspired computing, with applications in health care, finance, surveillance, manufacturing, robotics, animal breeding, etc. \end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/Petia-foto.jpg}}]{Dr. Petia Radeva}
is a senior researcher and associate professor at the University of Barcelona. She is Head of Computer Vision at University of Barcelona group and the MiLab of Computer Vision Center. Her present research interests are on development of learning-based approaches for computer vision, egocentric vision and medical imaging.
\end{IEEEbiography}


==> extra.tex <==
\ifCLASSOPTIONcompsoc
  \section*{Acknowledgments}

\else
  \section*{Acknowledgment}
  This work was partially founded by Ministerio de Ciencia e Innovaci\'on of the Gobierno de Espa\~na, through the research project TIN2015-66951-C2. SGR 1742, CERCA,  Nestore Horizon2020 SC1-PM-15-2017 (n° 769643), \textit{ICREA Academia 2014} and Grant 20141510 (Marat\'{o} TV3). The founders had no role in the study design, data collection, analysis, and preparation of the manuscript. The authors gratefully acknowledge the support of NVIDIA Corporation with the donation of the Titan Xp GPU used for this research. The data collected as part of the study and given labels is publicly available from the research group's website: \url{http://www.ub.edu/cvub/dataset/}

\fi
\ifCLASSOPTIONcaptionsoff
  \newpage
\fi

==> splitDataset.tex <==
\resizebox{0.9\textwidth}{!}{\begin{tabular}{c|ccccccccccccccc|c}
Categories 
 & \begin{rotate}{45} bakery shop \end{rotate}
 & \begin{rotate}{45} bar \end{rotate}
 & \begin{rotate}{45} beer hall \end{rotate}
 & \begin{rotate}{45} pub indoor \end{rotate}
 & \begin{rotate}{45} cafeteria \end{rotate}
 & \begin{rotate}{45} coffee shop \end{rotate}
 & \begin{rotate}{45} dining room \end{rotate}
 & \begin{rotate}{45} food court \end{rotate}
 & \begin{rotate}{45} ice-cream shop \end{rotate}
 & \begin{rotate}{45} kitchen \end{rotate}
 & \begin{rotate}{45} market indoor \end{rotate}
 & \begin{rotate}{45} market outdoor \end{rotate}
 & \begin{rotate}{45} picnic area \end{rotate}
 & \begin{rotate}{45} restaurant \end{rotate}
 & \begin{rotate}{45} supermarket \end{rotate}
 & \begin{rotate}{45} Num Images \end{rotate} \\ \hline \hline
Images Class & 342 & 1632 & 926 & 1383 & 666 & 2920 & 3639 & 1057 & 107 & 3835 &1731  & 1245 & 1608 & 7105 & 5607 & 33803 \\ \hline
Training & 301  & 1126 & 568 & 1198 & 175  & 2219 & 2636 & 1032 & 70 & 2660 & 1421  & 661 & 1348 & 4001 & 4195 & 23611 \\ \hline
Validation & 14 & 181 & 296 & 45 & 178 & 212 & 295 & 18 & 12 & 415  & 89 & 488 & 87 & 1105 & 498 & 3933 \\ \hline
Test & 27 & 325 & 62 & 140 & 313 & 489 & 708 & 7 & 25 & 760 & 221 & 96 & 173 & 1999 & 914 & 6259 \\ \hline
\end{tabular}}


\begin{comment}
% total
342, 1632, 926, 1383, 666, 2920, 3639, 1057, 107, 3835, 1731, 1245, 1608, 7105, 5607
%train
[ 301, 1126,  568, 1198,  175, 2219, 2636, 1032,   70, 2660, 1421,
         661, 1348, 4001, 4195]
% validation 
[  14,  181,  296,   45,  178,  212,  295,   18,   12,  415,   89,
         488,   87, 1105,  498]
          
% [  27,  325,   62,  140,  313,  489,  708,    7,   25,  760,  221,
          96,  173, 1999,  914])
\end{comment}

==> tabAverageResults.tex <==
\begin{tabular}{c|cccccccc}
 & OurModel & FV & Tree+SVM & RF & SVM & KNN & MACNet\cite{sarker2018macnet} & EnsembleFV\\ \hline \hline
Macro Precision & 0.57 & 0.54 & 0.56 & 0.59 & 0.56 & 0.58 & 0.47 & \\

Macro Recall & 0.52 & 0.51 & 0.50 & 0.47 & 0.50 & 0.48 & 0.48 & \\ \hline 

Macro Fscore & 0.52 & 0.49 & 0.50 & 0.48 & 0.50 & 0.49 & 0.44& \\ \hline \hline

Accuracy & 0.70 & 0.69 & 0.69 & 0.69 & 0.69 & 0.69 & 0.66 &  \\ \hline \hline

Weighted Precision & 0.69 & 0.68 & 0.68 & 0.68 & 0.68 & 0.68 & 0.66 & \\

Weighted Recall & 0.70 & 0.69 & 0.69 & 0.69 & 0.69 & 0.69 & 0.66 & \\ \hline 

Weighted Fscore & 0.68 & 0.66 & 0.67 & 0.66 & 0.66 & 0.66 & 0.65 & \\ \hline \hline
\end{tabular}

\begin{comment}


\begin{tabular}{c|ccccccc}
 & OurModel & FV & Tree+SVM & RF & SVM & KNN & MACNet \\ \hline \hline
Macro Precision & 0.57$\pm$0.01 & 0.54$\pm$0.02 & 0.56$\pm$0.01 & 0.59$\pm$0.01 & 0.56$\pm$0.01 & 0.58$\pm$0.02 & 0.47$\pm$0.03 \\

Macro Recall & 0.52$\pm$0.02 & 0.51$\pm$0.04 & 0.50$\pm$0.04 & 0.47$\pm$0.05 & 0.50$\pm$0.05 & 0.48$\pm$0.04 & 0.48$\pm$0.03 \\ \hline 

Macro Fscore & 0.52$\pm$0.04 & 0.49$\pm$0.04 & 0.50$\pm$0.04 & 0.48$\pm$0.04 & 0.50$\pm$0.05 & 0.49$\pm$0.04 & 0.44$\pm$0.04\\ \hline \hline

Accuracy & 0.70$\pm$0.03 & 0.69$\pm$0.04 & 0.69$\pm$0.04 & 0.69$\pm$0.05 & 0.69$\pm$0.04 & 0.69$\pm$0.05 & 0.66$\pm$0.04 \\ \hline \hline

Weighted Precision & 0.69$\pm$0.04 & 0.68$\pm$0.06 & 0.68$\pm$0.06 & 0.68$\pm$0.06 & 0.68$\pm$0.06 & 0.68$\pm$0.06 & 0.66$\pm$0.06 \\

Weighted Recall & 0.70$\pm$0.03 & 0.69$\pm$0.04 & 0.69$\pm$0.04 & 0.69$\pm$0.05 & 0.69$\pm$0.04 & 0.69$\pm$0.05 & 0.66$\pm$0.04 \\ \hline 

Weighted Fscore & 0.68$\pm$0.04 & 0.66$\pm$0.05 & 0.67$\pm$0.05 & 0.66$\pm$0.06 & 0.66$\pm$0.06 & 0.66$\pm$0.06 & 0.65$\pm$0.05 \\ \hline \hline
\end{tabular}
\end{comment}


==> tableLayersTree.tex <==
\setlength\tabcolsep{3.7pt}

\begin{tabular}{c|ccc|cc|}
 & Eating & Preparing & Acquiring & Acc &  W-Acc \\ \hline 
L1 & 94.11  & 95.13 & 94.5 & 94.31 & 94.58 \\ \hline \hline
\end{tabular}

\vspace{4mm}

\begin{tabular}{c|cc|c|cc|cc|}
 & Outdoor & Indoor & Kitchen & Self-Service & Attended & Acc &  W-Acc  \\ \hline  
L2  & 94.00  & 0.00  & 95.13  & 93.00 & 44.00 & 90.04 & 93.60\\ \hline \hline
\end{tabular}

\begin{comment}
\begin{tabular}{c|cc|cc|}
 & Outdoor & Indoor & Acc &  W-Acc  \\ \hline  
L 2-a  & 0.0 & 100 & 95.89 & 0.5\\ \hline \hline
\end{tabular}

\vspace{2mm}

\begin{tabular}{c|cc|cc|}
 & Self-Service & Attended & Acc &  W-Acc \\ \hline 
L 2-b & 96.21 & 55.48 & 91.32 & 75.85 \\ \hline \hline
\end{tabular}

%-------------------------------------------------

\begin{tabular}{c|ccccccc|cc|}
 & \begin{rotate}{78} Bar \end{rotate}
 & \begin{rotate}{78} Beer hall \end{rotate}
 & \begin{rotate}{78} Pub indoor \end{rotate}
 & \begin{rotate}{78} Cafeteria \end{rotate}
 & \begin{rotate}{78} Coffee shop \end{rotate}
 & \begin{rotate}{78} Dining room \end{rotate}
 & \begin{rotate}{78} Restaurant \end{rotate}
 & Acc & W-Acc \\ \hline
L 3-c  & 75.86 & 82.64 & 77.0 & 66.05 & 35.38 & 84.29 & 91.94 & 75.22 & 73.16\\ \hline \hline
\end{tabular}
\vspace{2mm}

\begin{tabular}{c|cc|cc|}
 & Supermarket & Market Ind & Acc & W-Acc \\ \hline 
L 3-d  & 97.92  & 83.26  & 95.06  & 90.58 \\ \hline \hline

\end{tabular}

\vspace{2mm}


\begin{tabular}{c|cccc|cc|}
 & Bakery & Food Court & Market Out & IceC shop & Acc & W-Acc  \\ \hline 
L 3-e & 70.37  & 71.43  & 94.79 & 64.0  & 84.52 & 75.15\\ \hline \hline
\end{tabular}

\end{comment}

\begin{comment}

 & \begin{rotate}{90} Bar \end{rotate}
 & \begin{rotate}{45} Beer hall \end{rotate}
 & \begin{rotate}{45} Pub indoor \end{rotate}
 & \begin{rotate}{45} Cafeteria \end{rotate}
 & \begin{rotate}{45} Coffee shop \end{rotate}
 & \begin{rotate}{45} Dining room \end{rotate}
 & \begin{rotate}{45} Restaurant \end{rotate}
 
 
 
 & \begin{rotate}{40} Bar \end{rotate}
 & \begin{rotate}{40} BeerH \end{rotate}
 & \begin{rotate}{40} PubI \end{rotate}
 & \begin{rotate}{40} Caft \end{rotate}
 & \begin{rotate}{40} Coffee shop \end{rotate}
 & \begin{rotate}{40} DininR \end{rotate}
 & \begin{rotate}{40} Rest \end{rotate}
\end{comment}

==> updatedArxiv-Food-related-Scenes-JBHI - Minor Revision - May/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> updatedArxiv-Food-related-Scenes-JBHI - Minor Revision - May/bayesian_example.tex <==
In order to understand the behaviour of the BSN model, we illustrate a simple example. Let us imagine that we have the semantic tree in Fig. \ref{fig:baynet}, and that we want to classify an egocentric image belonging to the class \textit{dining room}. In order to classify the given image, we compute the probability of the images belonging to the classes at the different levels of the semantic tree. First, we obtain the classification probabilities of the classes $P(eating)$, $P(shopping)$, and $P(preparing)$, corresponding to categories in Level 1 of the semantic tree (see Fig. \ref{fig:baynet}). In the second step, we obtain the classification probabilities with respect to the classes in Level 2. Finally, the probabilities of the classes included in  Level 3.  Our sample image describes the class \textit{dining room}. Thus, from the different levels classifications, we expect that the highest probabilities correspond to the category \textit{eating}, $P(indoor|eating)$ and $P(dining room|indoor)$, at Level 1, Level 2 and Level 3, respectively. 


Let us consider classes $C^i$ and $C^{i-1}$ so that subindex shows the level of the class in the hierarchy and $C^{i-1}$ is parent of $C^i$ in the higher level in the hierarchical organization of the tree.  

\begin{equation}
\resizebox{.3\textwidth}{!} 
{
$P(Q|C^{i-1}) = \frac{P(C^{i-1}|C^i)*P(C^i)}{P(C^{i-1})}$
}
\end{equation} or
\begin{equation}
\resizebox{.3\textwidth}{!} 
{
$P(C^i) = \frac{P(C^i|C^{i-1})*P(C^{i-1})}{P(C^{i-1}|C^i)}$
}
\end{equation}
Note that we can estimate $P(Q|C^{i-1})$ from the classifier of the network trained to classify the classes children of class $Q$, $P(C^{i-1}|C^i)$ is 1 since $C^i$ is a subclass of $C^{i-1}$  and $P(C^{i-1})$ is recursively estimated by applying the Bayes rule on $C^{i-1}$ and its class parent. 
\begin{equation}
\resizebox{.3\textwidth}{!} 
{
$P(C^i) = P(C^i|C^{i-1})*P(C^{i-1})$
}
\end{equation}
Applying recursively the Bayes rule, we obtain that 
\begin{equation}
\resizebox{.4\textwidth}{!} 
{
$P(C^i) = \Pi_{j=1}`^i P(C^j|C^{j-1})*P(C^{j-1})$
}
\end{equation}
Without loss of generality, we consider that the probability of the class in the root is 1 ($P(C^0)$). 

\textcolor{red}{De hecho esto es falso!!!! Para que sea aplicable, no necesitamos en la raiz un clasificador de food-related vs no food related?}

\textcolor{red}{Dejar numeros solo en las ecuaciones que se citan}

Let us illustrate this process on an example:
%\noindent At the same time, following the semantic tree, we know that:
\begin{equation}
\resizebox{.3\textwidth}{!} 
{
$P(indoor|eating) = \frac{P(eating|indoor)*P(indoor)}{P(eating)}$
}
\end{equation}
\begin{equation}
\resizebox{.3\textwidth}{!} 
{
$P(indoor) = \frac{P(eating)*P(indoor|eating)}{P(eating|indoor)}$
}
\end{equation}


Following the Bayes' theorem, we state that:
\begin{equation}
\resizebox{.4\textwidth}{!} 
{
$P(dining room|indoor) = \frac{P(indoor|dining room)*P(dining room)}{P(indoor)}$
}
\end{equation}
\begin{equation}
\resizebox{.3\textwidth}{!} 
{
$P(dining room) = \frac{P(indoor)*P(dining room|indoor)}{P(indoor|dining room)}$
}
\end{equation}
\noindent At the same time, following the semantic tree, we know that:
\begin{equation}
\resizebox{.3\textwidth}{!} 
{
$P(indoor|eating) = \frac{P(eating|indoor)*P(indoor)}{P(eating)}$
}
\end{equation}
\begin{equation}
\resizebox{.3\textwidth}{!} 
{
$P(indoor) = \frac{P(eating)*P(indoor|eating)}{P(eating|indoor)}$
}
\end{equation}

\noindent Thus, we can combine the probabilities and get the following equation that relates the probability of the events occurring,
\begin{equation}
\resizebox{.45\textwidth}{!} 
{
$P(dining room) =  \frac{P(dining room|indoor)*P(eating)*P(indoor|eating)}{P(eating|indoor)*P(indoor|dining room)}$
}
\end{equation}
 
%%%%
\noindent By having a look at the semantic tree defined, we know that \textit{indoor} relates to \textit{eating}, as \textit{dining room} relates to \textit{indoor eating}. Therefore, $P(eating|indoor)$ and $P(indoor|diningRoom)$ are equal to $1$. The probability of Dining Room occurring can be computed as:
\begin{equation}
\resizebox{.5\textwidth}{!} 
{
$P(dining room) =  P(dining room|indoor)*P(eating)*P(indoor|eating)$
}
\end{equation}

\begin{comment}
Furthermore, following this methodology we could assume and analyse several other aspects. For instance, we could go further and infer the probability of being at home eating as $P(home)$:
\begin{equation}
\resizebox{.3\textwidth}{!} 
{
$P(home|diningR) = \frac{P(diningR|home)*P(home)}{P(diningR)} = $
}
\end{equation}
\begin{equation}
\resizebox{.3\textwidth}{!} 
{
$\quad = P(home|diningR)*P(diningR|indoor)*P(indoor) $
}
\end{equation}
\end{comment}

To summarize, given an image our proposed BSN model computes the final classification by combining the obtained classification probabilities at the different levels of the defined semantic tree, following the Bayes’ theorem. 


==> updatedArxiv-Food-related-Scenes-JBHI - Minor Revision - May/bibliographies.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/foto_perfil_EstefaniaTalavera.png}}]{Estefania Talavera}
received her BSc degree in electronic engineering from Balearic Islands University in 2012 and her MSc degree in biomedical engineering from Polytechnic University of Catalonia in 2014. She is currently a PhD student at the University of Barcelona and University of Groningen. Her research interests are lifelogging and health applications.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/foto_maria.jpg}}]{María Leyva} received her BSc degree in Software Engineering from the University of Oviedo in 2011. She continued her studies with the MSc in Artificial Intelligence in the Polytechnic University of Catalonia, graduating in 2017. She is currently a PhD Student at the Johann Bernoulli Institute for Mathematics and Computer Science in the University of Groningen. \end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/Petia-foto.jpg}}]{Mostafa Kamal}
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/NicolaiPetkov.png}}]{Prof. Nicolai Petkov} received Dr.sc.techn. degree in Computer Engineering (Informationstechnik) from Dresden University of Technology, Dresden, Germany. Since 1991, he is professor of computer science and head of the Intelligent Systems group. His current research is in pattern recognition, machine learning, data analytics and brain-inspired computing, with applications in health care, finance, surveillance, manufacturing, robotics, animal breeding, etc. \end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/Petia-foto.jpg}}]{Dr. Petia Radeva}
is a senior researcher and associate professor at the University of Barcelona. She is Head of Computer Vision at University of Barcelona group and the MiLab of Computer Vision Center. Her present research interests are on development of learning-based approaches for computer vision, egocentric vision and medical imaging.
\end{IEEEbiography}


==> updatedArxiv-Food-related-Scenes-JBHI - Minor Revision - May/extra.tex <==
\ifCLASSOPTIONcompsoc
  \section*{Acknowledgments}

\else
  \section*{Acknowledgment}
  This work was partially founded by Ministerio de Ciencia e Innovaci\'on of the Gobierno de Espa\~na, through the research project TIN2015-66951-C2. SGR 1742, CERCA,  Nestore Horizon2020 SC1-PM-15-2017 (n° 769643), \textit{ICREA Academia 2014} and Grant 20141510 (Marat\'{o} TV3). The founders had no role in the study design, data collection, analysis, and preparation of the manuscript. The authors gratefully acknowledge the support of NVIDIA Corporation with the donation of the Titan Xp GPU used for this research. The data collected as part of the study and given labels is publicly available from the research group's website: \url{http://www.ub.edu/cvub/dataset/}

\fi
\ifCLASSOPTIONcaptionsoff
  \newpage
\fi

==> updatedArxiv-Food-related-Scenes-JBHI - Minor Revision - May/figure_t-sne.tex <==

\begin{comment}
\minipage{0.4\textwidth}
\includegraphics[width=0.6\textwidth]{Figures/train_t-sne.png}
\endminipage\hfill
\minipage{0.4\textwidth}
\includegraphics[width=0.8\textwidth]{Figures/test_t-sne.png} 
\endminipage\hfill
\minipage{0.2\textwidth}%
\centering
\includegraphics[width=.7\textwidth]{Figures/legend_t-sne.png}
\endminipage
\end{comment}

%\includegraphics[width=.65\linewidth]{Figures/train_t-sne.png}
\includegraphics[width=\linewidth]{Figures/testsamples_trainTSNE.png}
%\includegraphics[width=.3\linewidth]{Figures/legend_t-sne.png}


==> updatedArxiv-Food-related-Scenes-JBHI - Minor Revision - May/splitDataset.tex <==
\resizebox{0.9\textwidth}{!}{\begin{tabular}{c|ccccccccccccccc|c}
Categories 
 & \begin{rotate}{45} bakery shop \end{rotate}
 & \begin{rotate}{45} bar \end{rotate}
 & \begin{rotate}{45} beer hall \end{rotate}
 & \begin{rotate}{45} pub indoor \end{rotate}
 & \begin{rotate}{45} cafeteria \end{rotate}
 & \begin{rotate}{45} coffee shop \end{rotate}
 & \begin{rotate}{45} dining room \end{rotate}
 & \begin{rotate}{45} food court \end{rotate}
 & \begin{rotate}{45} ice-cream shop \end{rotate}
 & \begin{rotate}{45} kitchen \end{rotate}
 & \begin{rotate}{45} market indoor \end{rotate}
 & \begin{rotate}{45} market outdoor \end{rotate}
 & \begin{rotate}{45} picnic area \end{rotate}
 & \begin{rotate}{45} restaurant \end{rotate}
 & \begin{rotate}{45} supermarket \end{rotate}
 & \begin{rotate}{45} Num Images \end{rotate} \\ \hline \hline
Images Class & 342 & 1632 & 926 & 1383 & 666 & 2920 & 3639 & 1057 & 107 & 3835 &1731  & 1245 & 1608 & 7105 & 5607 & 33803 \\ \hline
Training & 301  & 1126 & 568 & 1198 & 175  & 2219 & 2636 & 1032 & 70 & 2660 & 1421  & 661 & 1348 & 4001 & 4195 & 23611 \\ \hline
Validation & 14 & 181 & 296 & 45 & 178 & 212 & 295 & 18 & 12 & 415  & 89 & 488 & 87 & 1105 & 498 & 3933 \\ \hline
Test & 27 & 325 & 62 & 140 & 313 & 489 & 708 & 7 & 25 & 760 & 221 & 96 & 173 & 1999 & 914 & 6259 \\ \hline
\end{tabular}}


\begin{comment}
% total
342, 1632, 926, 1383, 666, 2920, 3639, 1057, 107, 3835, 1731, 1245, 1608, 7105, 5607
%train
[ 301, 1126,  568, 1198,  175, 2219, 2636, 1032,   70, 2660, 1421,
         661, 1348, 4001, 4195]
% validation 
[  14,  181,  296,   45,  178,  212,  295,   18,   12,  415,   89,
         488,   87, 1105,  498]
          
% [  27,  325,   62,  140,  313,  489,  708,    7,   25,  760,  221,
          96,  173, 1999,  914])
\end{comment}

==> updatedArxiv-Food-related-Scenes-JBHI - Minor Revision - May/tabAverageResults.tex <==
\begin{tabular}{c|cccccccc}
 & OurModel & FV & Tree+SVM & RF & SVM & KNN & MACNet\cite{sarker2018macnet} & EnsembleFV\\ \hline \hline
Macro Precision & 0.57 & 0.54 & 0.56 & 0.59 & 0.56 & 0.58 & 0.47 & \\

Macro Recall & 0.52 & 0.51 & 0.50 & 0.47 & 0.50 & 0.48 & 0.48 & \\ \hline 

Macro Fscore & 0.52 & 0.49 & 0.50 & 0.48 & 0.50 & 0.49 & 0.44& \\ \hline \hline

Accuracy & 0.70 & 0.69 & 0.69 & 0.69 & 0.69 & 0.69 & 0.66 &  \\ \hline \hline

Weighted Precision & 0.69 & 0.68 & 0.68 & 0.68 & 0.68 & 0.68 & 0.66 & \\

Weighted Recall & 0.70 & 0.69 & 0.69 & 0.69 & 0.69 & 0.69 & 0.66 & \\ \hline 

Weighted Fscore & 0.68 & 0.66 & 0.67 & 0.66 & 0.66 & 0.66 & 0.65 & \\ \hline \hline
\end{tabular}

\begin{comment}


\begin{tabular}{c|ccccccc}
 & OurModel & FV & Tree+SVM & RF & SVM & KNN & MACNet \\ \hline \hline
Macro Precision & 0.57$\pm$0.01 & 0.54$\pm$0.02 & 0.56$\pm$0.01 & 0.59$\pm$0.01 & 0.56$\pm$0.01 & 0.58$\pm$0.02 & 0.47$\pm$0.03 \\

Macro Recall & 0.52$\pm$0.02 & 0.51$\pm$0.04 & 0.50$\pm$0.04 & 0.47$\pm$0.05 & 0.50$\pm$0.05 & 0.48$\pm$0.04 & 0.48$\pm$0.03 \\ \hline 

Macro Fscore & 0.52$\pm$0.04 & 0.49$\pm$0.04 & 0.50$\pm$0.04 & 0.48$\pm$0.04 & 0.50$\pm$0.05 & 0.49$\pm$0.04 & 0.44$\pm$0.04\\ \hline \hline

Accuracy & 0.70$\pm$0.03 & 0.69$\pm$0.04 & 0.69$\pm$0.04 & 0.69$\pm$0.05 & 0.69$\pm$0.04 & 0.69$\pm$0.05 & 0.66$\pm$0.04 \\ \hline \hline

Weighted Precision & 0.69$\pm$0.04 & 0.68$\pm$0.06 & 0.68$\pm$0.06 & 0.68$\pm$0.06 & 0.68$\pm$0.06 & 0.68$\pm$0.06 & 0.66$\pm$0.06 \\

Weighted Recall & 0.70$\pm$0.03 & 0.69$\pm$0.04 & 0.69$\pm$0.04 & 0.69$\pm$0.05 & 0.69$\pm$0.04 & 0.69$\pm$0.05 & 0.66$\pm$0.04 \\ \hline 

Weighted Fscore & 0.68$\pm$0.04 & 0.66$\pm$0.05 & 0.67$\pm$0.05 & 0.66$\pm$0.06 & 0.66$\pm$0.06 & 0.66$\pm$0.06 & 0.65$\pm$0.05 \\ \hline \hline
\end{tabular}
\end{comment}


==> updatedArxiv-Food-related-Scenes-JBHI - Minor Revision - May/tab_metaclasses.tex <==
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc|}
 & \multicolumn{2}{c|}{Our Method} & \multicolumn{2}{c|}{FV} & \multicolumn{2}{c|}{SVMTree} & \multicolumn{2}{c|}{FV+RF} & \multicolumn{2}{c|}{FV+SVM} & \multicolumn{2}{c|}{FV+KNN} & \multicolumn{2}{c|}{MACNet\cite{sarker2018macnet}} & \multicolumn{2}{c|}{EnsembleCNN} \\ \cline{2-17} 
 & Acc & WAcc & Acc & WAcc & Acc & WAcc & Acc & WAcc & Acc & WAcc & Acc & WAcc & Acc & WAcc& Acc & WAcc \\ \hline \hline
\multicolumn{1}{|c|}{Level 1 (L1)} & \textbf{0.944} & \textbf{0.947} & 0.927 & 0.919 & 0.934 & 0.931 & 0.928 & 0.922 & 0.927 & 0.924 & 0.927 & 0.910 & 0.884 & 0.865 & 0.923 & 0.913\\
\multicolumn{1}{|c|}{Level 2a (L2a)} & \textbf{0.915} & \textbf{0.685} & 0.886 & 0.664 & 0.898 & 0.673 & 0.890 & 0.666 & 0.800 & 0.753 & 0.890 & 0.648 & 0.829 & 0.623& 0.869 & 0.629 \\
\multicolumn{1}{|c|}{Level 2b (L2b)} & \textbf{0.893} & \textbf{0.947} & 0.890 & 0.940 & 0.890 & 0.944 & 0.885 & 0.945 & 0.897 & 0.935 & 0.885 & 0.927 & 0.860 & 0.906 & 0.856  & \textbf{0.955}\\ \hline \hline
\end{tabular}}

\begin{comment}


\begin{tabular}{cccccccccccccc}
& & \multicolumn{2}{c}{ Our Method } & \multicolumn{2}{c}{ FV } & \multicolumn{2}{c}{ SVMTree } & \multicolumn{2}{c}{ FV+RF } & \multicolumn{2}{c}{ FV+SVM } & \multicolumn{2}{c}{ FV+KNN } \\
& & Acc & WAcc & Acc & WAcc & Acc & WAcc & Acc & WAcc & Acc & WAcc & Acc & WAcc \\
\multirow{3}{*}{ Fold 1 } & Level 1 (L1) & 0.945 & 0.957 & 0.916 & 0.921 & 0.923 & 0.930 & 0.922 & 0.927 & 0.916 & 0.920 & 0.917 & 0.922 \\
& Level 2a (L2a) & 0.920 & 0.625 & 0.892 & 0.606 & 0.899 & 0.610 & 0.896 & 0.609 & 0.887 & 0.602 & 0.892 & 0.606 \\
& Level 2b (L2b) & 0.833 & 0.891 & 0.846 & 0.901 & 0.846 & 0.904 & 0.846 & 0.911 & 0.845 & 0.903 & 0.845 & 0.906 \\
\multirow{3}{*}{ Fold 2 } & Level 1 (L1) & 0.928 & 0.923 & 0.897 & 0.881 & 0.907 & 0.896 & 0.896 & 0.880 & 0.897 & 0.881 & 0.897 & 0.882 \\
& Level 2a (L2a) & 0.880 & 0.637 & 0.840 & 0.608 & 0.855 & 0.619 & 0.838 & 0.606 & 0.838 & 0.607 & 0.842 & 0.609 \\
& Level 2b (L2b) & 0.844 & 0.949 & 0.847 & 0.943 & 0.847 & 0.947 & 0.843 & 0.950 & 0.844 & 0.945 & 0.836 & 0.939 \\
\multirow{3}{*}{ Fold 3 } & Level 1 (L1) & 0.938 & 0.950 & 0.924 & 0.931 & 0.931 & 0.942 & 0.922 & 0.928 & 0.927 & 0.935 & 0.923 & 0.930 \\
& Level 2a (L2a) & 0.916 & 0.652 & 0.896 & 0.637 & 0.909 & 0.646 & 0.892 & 0.634 & 0.900 & 0.640 & 0.895 & 0.636 \\
& Level 2b (L2b) & 0.920 & 0.944 & 0.915 & 0.938 & 0.917 & 0.940 & 0.916 & 0.947 & 0.920 & 0.943 & 0.920 & 0.947 \\
\multirow{3}{*}{ Fold 4 } & Level 1 (L1) & 0.929 & 0.951 & 0.910 & 0.915 & 0.917 & 0.927 & 0.903 & 0.907 & 0.910 & 0.915 & 0.901 & 0.904 \\
& Level 2a (L2a) & 0.920 & 0.639 & 0.874 & 0.608 & 0.887 & 0.616 & 0.864 & 0.600 & 0.873 & 0.607 & 0.861 & 0.599 \\
& Level 2b (L2b) & 0.869 & 0.925 & 0.894 & 0.929 & 0.894 & 0.932 & 0.888 & 0.944 & 0.893 & 0.934 & 0.891 & 0.931 \\
\multirow{3}{*}{ Fold 5 } & Level 1 (L1) & 0.943 & 0.943 & 0.930 & 0.922 & 0.934 & 0.930 & 0.930 & 0.926 & 0.928 & 0.933 & 0.928 & 0.923 \\
& Level 2a (L2a) & 0.903 & 0.633 & 0.882 & 0.619 & 0.890 & 0.625 & 0.887 & 0.622 & 0.622 & 0.887 & 0.886 & 0.622 \\
& Level 2b (L2b) & 0.912 & 0.936 & 0.908 & 0.930 & 0.909 & 0.933 & 0.902 & 0.934 & 0.932 & 0.909 & 0.902 & 0.929 \\
\multirow{3}{*}{ fold70 } & Level 1 (L1) & 0.941 & 0.940 & 0.895 & 0.890 & 0.901 & 0.904 & 0.894 & 0.890 & 0.892 & 0.887 & 0.897 & 0.891 \\
& Level 2a (L2a) & 0.930 & 0.800 & 0.868 & 0.747 & 0.758 & 0.881 & 0.866 & 0.745 & 0.863 & 0.743 & 0.872 & 0.750 \\
& Level 2b (L2b) & 0.869 & 0.925 & 0.867 & 0.933 & 0.940 & 0.873 & 0.877 & 0.950 & 0.871 & 0.944 & 0.861 & 0.933 \\
\multirow{3}{*}{ fold70-1 } & Level 1 (L1) & 0.932 & 0.937 & 0.908 & 0.913 & 0.923 & 0.927 & 0.899 & 0.909 & 0.910 & 0.914 & 0.902 & 0.906 \\
& Level 2a (L2a) & 0.909 & 0.785 & 0.878 & 0.767 & 0.899 & 0.760 & 0.867 & 0.741 & 0.880 & 0.756 & 0.875 & 0.756 \\
& Level 2b (L2b) & 0.907 & 0.929 & 0.909 & 0.928 & 0.909 & 0.928 & 0.909 & 0.932 & 0.913 & 0.932 & 0.906 & 0.923 \\
\multirow{3}{*}{ fold80 } & Level 1 (L1) & 0.963 & 0.974 & 0.954 & 0.954 & 0.959 & 0.965 & 0.957 & 0.961 & 0.956 & 0.957 & 0.955 & 0.926 \\
& Level 2a (L2a) & 0.963 & 0.785 & 0.937 & 0.764 & 0.950 & 0.775 & 0.945 & 0.771 & 0.940 & 0.766 & 0.943 & 0.712 \\
& Level 2b (L2b) & 0.924 & 0.956 & 0.916 & 0.948 & 0.915 & 0.951 & 0.910 & 0.952 & 0.915 & 0.952 & 0.916 & 0.913 \\
\multirow{3}{*}{ fold80-1 } & Level 1 (L1) & 0.948 & 0.943 & 0.922 & 0.905 & 0.931 & 0.921 & 0.939 & 0.931 & 0.927 & 0.914 & 0.933 & 0.926 \\
& Level 2a (L2a) & 0.924 & 0.721 & 0.890 & 0.699 & 0.907 & 0.708 & 0.916 & 0.714 & 0.898 & 0.701 & 0.913 & 0.712 \\
& Level 2b (L2b) & 0.814 & 0.935 & 0.785 & 0.916 & 0.782 & 0.914 & 0.781 & 0.917 & 0.787 & 0.920 & 0.779 & 0.913 \\ \hline
\end{tabular}
\end{comment}

==> updatedArxiv-Food-related-Scenes-JBHI - Minor Revision - May/tableLayersTree.tex <==
\setlength\tabcolsep{3.7pt}

\begin{tabular}{c|ccc|cc|}
 & Eating & Preparing & Acquiring & Acc &  W-Acc \\ \hline 
L1 & 94.11  & 95.13 & 94.5 & 94.31 & 94.58 \\ \hline \hline
\end{tabular}

\vspace{4mm}

\begin{tabular}{c|cc|c|cc|cc|}
 & Outdoor & Indoor & Kitchen & Self-Service & Attended & Acc &  W-Acc  \\ \hline  
L2  & 94.00  & 0.00  & 95.13  & 93.00 & 44.00 & 90.04 & 93.60\\ \hline \hline
\end{tabular}

\begin{comment}
\begin{tabular}{c|cc|cc|}
 & Outdoor & Indoor & Acc &  W-Acc  \\ \hline  
L 2-a  & 0.0 & 100 & 95.89 & 0.5\\ \hline \hline
\end{tabular}

\vspace{2mm}

\begin{tabular}{c|cc|cc|}
 & Self-Service & Attended & Acc &  W-Acc \\ \hline 
L 2-b & 96.21 & 55.48 & 91.32 & 75.85 \\ \hline \hline
\end{tabular}

%-------------------------------------------------

\begin{tabular}{c|ccccccc|cc|}
 & \begin{rotate}{78} Bar \end{rotate}
 & \begin{rotate}{78} Beer hall \end{rotate}
 & \begin{rotate}{78} Pub indoor \end{rotate}
 & \begin{rotate}{78} Cafeteria \end{rotate}
 & \begin{rotate}{78} Coffee shop \end{rotate}
 & \begin{rotate}{78} Dining room \end{rotate}
 & \begin{rotate}{78} Restaurant \end{rotate}
 & Acc & W-Acc \\ \hline
L 3-c  & 75.86 & 82.64 & 77.0 & 66.05 & 35.38 & 84.29 & 91.94 & 75.22 & 73.16\\ \hline \hline
\end{tabular}
\vspace{2mm}

\begin{tabular}{c|cc|cc|}
 & Supermarket & Market Ind & Acc & W-Acc \\ \hline 
L 3-d  & 97.92  & 83.26  & 95.06  & 90.58 \\ \hline \hline

\end{tabular}

\vspace{2mm}


\begin{tabular}{c|cccc|cc|}
 & Bakery & Food Court & Market Out & IceC shop & Acc & W-Acc  \\ \hline 
L 3-e & 70.37  & 71.43  & 94.79 & 64.0  & 84.52 & 75.15\\ \hline \hline
\end{tabular}

\end{comment}

\begin{comment}

 & \begin{rotate}{90} Bar \end{rotate}
 & \begin{rotate}{45} Beer hall \end{rotate}
 & \begin{rotate}{45} Pub indoor \end{rotate}
 & \begin{rotate}{45} Cafeteria \end{rotate}
 & \begin{rotate}{45} Coffee shop \end{rotate}
 & \begin{rotate}{45} Dining room \end{rotate}
 & \begin{rotate}{45} Restaurant \end{rotate}
 
 
 
 & \begin{rotate}{40} Bar \end{rotate}
 & \begin{rotate}{40} BeerH \end{rotate}
 & \begin{rotate}{40} PubI \end{rotate}
 & \begin{rotate}{40} Caft \end{rotate}
 & \begin{rotate}{40} Coffee shop \end{rotate}
 & \begin{rotate}{40} DininR \end{rotate}
 & \begin{rotate}{40} Rest \end{rotate}
\end{comment}

==> updatedArxiv-Food-related-Scenes-JBHI - Minor Revision - May/table_acc_results.tex <==

\begin{tabular}{c|c|ccccccc}
& OurModel & FV & Tree+SVM & FV+RF & FV+SVM & FV+KNN & MACNet\cite{sarker2018macnet} & EnsembleCNNs \\  \hline \hline
bakery shop & 0.39 & 0.58 & 0.58 & 0.56 & 0.58 & 0.59 & 0.58 & 0.60 \\\hline
bar & 0.31 & 0.13 & 0.15 & 0.11 & 0.11 & 0.17 & 0.17 & 0.15 \\\hline
beer hall & 0.89 & 0.32 & 0.20 & 0.18 & 0.20 & 0.20 & 0.61 & 0.56 \\\hline
pub indoor & 0.85 & 0.70 & 0.71 & 0.71 & 0.71 & 0.71 & 0.64 & 0.82 \\\hline
cafeteria & 0.45 & 0.45 & 0.44 & 0.43 & 0.44 & 0.43 & 0.72 & 0.55 \\\hline
coffee shop & 0.59 & 0.40 & 0.39 & 0.34 & 0.38 & 0.34 & 0.49 & 0.49 \\\hline
dining room & 0.58 & 0.58 & 0.59 & 0.58 & 0.58 & 0.57 & 0.56 & 0.57 \\\hline
food court & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\\hline
ice-cream parlor & 0.52 & 0.59 & 0.68 & 0.65 & 0.64 & 0.65 & 0.15 & 0.73 \\\hline
kitchen & 0.89 & 0.87 & 0.89 & 0.87 & 0.86 & 0.86 & 0.88 & 0.90 \\\hline
market indoor & 0.70 & 0.73 & 0.76 & 0.77 & 0.77 & 0.76 & 0.66 & 0.77 \\\hline
market outdoor & 0.28 & 0.20 & 0.20 & 0.20 & 0.20 & 0.19 & 0.23 & 0.25 \\\hline
picnic area & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\\hline
restaurant & 0.70 & 0.67 & 0.68 & 0.68 & 0.68 & 0.68 & 0.63 & 0.73 \\\hline
supermarket & 0.85 & 0.81 & 0.81 & 0.79 & 0.81 & 0.80 & 0.75 & 0.84 \\  \hline \hline
Macro Precision & 0.56 & 0.53 & 0.55 & 0.59 & 0.55 & 0.56 & 0.48 & 0.60 \\\hline
Macro Recall & 0.53 & 0.48 & 0.47 & 0.44 & 0.46 & 0.45 & 0.49 & 0.52 \\\hline
Macro F1 & 0.53 & 0.47 & 0.47 & 0.46 & 0.46 & 0.46 & 0.47 & 0.53 \\  \hline \hline
Weighted Precision & 0.65 & 0.62 & 0.62 & 0.62 & 0.62 & 0.61 & 0.61 & 0.67 \\\hline
Weighted Recall & 0.68 & 0.64 & 0.64 & 0.64 & 0.64 & 0.64 & 0.63 & 0.68 \\\hline
Weighted F1 & 0.65 & 0.61 & 0.61 & 0.60 & 0.61 & 0.60 & 0.61 & 0.65 \\ \hline \hline
Accuracy & 0.68 & 0.64 & 0.64 & 0.64 & 0.64 & 0.64 & 0.63 & 0.68 \\\hline
Weighted Accuracy & 0.56 & 0.53 & 0.51 & 0.47 & 0.50 & 0.48 & 0.49 & 0.55 \\ \hline \hline
\end{tabular}


\begin{comment}


\resizebox{0.5\textwidth}{!}{ 
\begin{tabular}{c|cccccc}
Categories & 
BSN & 
FV & 
FV+RF & 
FV+KNN & 
FV+SVM 
& MACNet\cite{sarker2018macnet}\\ \hline \hline
bakery shop & \textbf{37.04} & 29.63 & 18.51 & 29.63 & 29.62 & 25.93 \\ \hline
bar & 33.54 & 25.85 & 22.77 & 25.54 & 26.77 & \textbf{42.77}\\ \hline
beer hall & 91.94 & 88.71 & 85.48 & 87.10 & 87.09 & \textbf{96.77}\\ \hline
pub indoor & \textbf{82.86} & \textbf{82.86} & 82.14 & \textbf{82.86} & 82.85 & 78.57\\ \hline
cafeteria & \textbf{73.80} & 58.47 & 54.95 & 56.87 & 59.10 & 59.10\\ \hline
coffee shop & 65.64 & 68.10 & 65.03 & 66.05 & 67.89 & \textbf{69.73}\\ \hline
dining room & 69.21 & \textbf{70.90} & 62.28 & 64.69 & 70.33 & 68.93\\ \hline
food court & \textbf{57.14} & 42.86 & 28.57 & 42.86 & 57.14 & 42.85 \\ \hline
ice cream parlor & 48.00 & \textbf{72.00} & 44.00 & 68.00 & \textbf{72.00} & 20.00\\ \hline
kitchen & 94.74 & 94.21 & 94.47 & 94.60 & 94.34 & \textbf{95.53}\\ \hline
market indoor & 77.38 & \textbf{78.28} & 70.14 & 72.40 & 76.92 & 61.09\\ \hline
market outdoor & \textbf{44.79} & 30.21 & 21.88 & 28.13 & 30.20 & 35.42\\ \hline
picnic area & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\ \hline
restaurant & 79.99 & 78.74 & 87.49 & \textbf{81.94} & 78.84 & 77.99\\ \hline
supermarket & 91.90 & 92.45 & \textbf{93.44} & 92.78 & 92.56 & 93.22\\ \hline \hline
Avg Acc. & \textbf{75.46} & 74.12 & 74.90 & 74.71 & 74.76 & 74.19 \\ \hline
Weigh Avg Acc. & \textbf{63.20} & 60.88 & 59.25 & 61.25 & 62.47 & 58.88\\ \hline \hline
\end{tabular}}

\end{comment}
\begin{comment}
MACNet

0 'bakery_shop',  0.259259259259
1 'bar', 0.427692307692
2 'beer_hall', 0.967741935484
3 'pub_indoor', 0.785714285714
4 'cafeteria', 0.591054313099
5 'coffee_shop', 0.697341513292
6 'dining_room', 0.689265536723
7'food_court', 0.428571428571
8 'ice_cream_parlor', 0.2
9 'kitchen', 0.955263157895
10 'market_indoor', 0.610859728507
11 'market_outdoor', 0.354166666667
12 'picnic_area', 0.0
13 'restaurant', 0.779889944972
14 'supermarket' 0.932166301969
             
\end{comment}







\begin{comment}
\begin{tabular}{c|cccccc}
Categories & 
BY-HC-FT & 
FT-VGG365 & 
HC-FT & 
FT-VGG365-RF & 
\multicolumn{1}{l}{FT-VGG365-KNN} & 
\multicolumn{1}{l}{FT-VGG365-SVM} \\ \hline \hline
bakery shop & 37.04 & 29.63 & 33.33 & 18.51 & 29.63 & 29.62 \\ \hline
bar & 33.54 & 25.85 & 0.62 & 22.77 & 25.54 & 26.77 \\ \hline
beer hall & 91.94 & 88.71 & 56.45 & 85.48 & 87.10 & 87.09 \\ \hline
pub indoor & 82.86 & 82.86 & 52.86 & 82.14 & 82.86 & 82.85 \\ \hline
cafeteria & 73.80 & 58.47 & 41.85 & 54.95 & 56.87 & 59.10 \\ \hline
coffee shop & 65.64 & 68.10 & 39.47 & 65.03 & 66.05 & 67.89 \\ \hline
dining room & 69.21 & 70.90 & 45.76 & 62.28 & 64.69 & 70.33 \\ \hline
food court & 57.14 & 42.86 & 57.14 & 28.57 & 42.86 & 57.14 \\ \hline
ice cream parlor & 48.00 & 72.00 & 20.00 & 44.00 & 68.00 & 72.00 \\ \hline
kitchen & 94.74 & 94.21 & 0.0 & 94.47 & 94.60 & 94.34 \\ \hline
market indoor & 77.38 & 78.28 & 40.27 & 70.14 & 72.40 & 76.92 \\ \hline
market outdoor & 44.79 & 30.21 & 71.88 & 21.88 & 28.13 & 30.20 \\ \hline
picnic area & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ \hline
restaurant & 79.99 & 78.74 & 37.02 & 87.49 & 81.94 & 78.84 \\ \hline
supermarket & 91.90 & 92.45 & 76.81 & 93.44 & 92.78 & 92.56 \\ \hline \hline
Avg Accuracy & 75.46 & 74.12 & 37.98 & 74.90 & 74.71 & 74.76 \\ \hline
Weighted Avg Accuracy & 63.20 & 60.88 & 38.23 & 59.25 & 61.25 & 62.47 \\ \hline \hline
\end{tabular}


Experimento sin priors
es maravillosamente malo
Top1 acc 0.379773126698 
Top1 weighted acc 0.382303089751 
Top3 acc 0.678383128295 
Top3 weighted acc 0.662617079007 
Top5 acc 0.779197954945 
Top5 weighted acc 0.762286504102
\end{comment}

\begin{comment}
Others
KNN 0.74053
SMV 0.7459
RF 0.74 (200) 0.732 (1)
RF (PCA) 0.7151 (200) 0.7055 (1)
RF (tSNE) 0.7103 (1)
RF (norm x=1) 0.7474 (200) 
RF (norm x=0) 0.7339 (200
\end{comment}
